RGB-Event ISP: The Dataset and Benchmark

Event-guided imaging has received significant attention due to its potential to revolutionize instant imaging systems. However, the prior methods primarily focus on enhancing RGB images in a post-processing manner, neglecting the challenges of image signal processor (ISP) dealing with event sensor and the benefits events provide for reforming the ISP process. To achieve this, we conduct the first research on event-guided ISP. First, we present a new event-RAW paired dataset, collected with a novel but still confidential sensor that records pixel-level aligned events and RAW images. This dataset includes 3373 RAW images with 2248 x 3264 resolution and their corresponding events, spanning 24 scenes with 3 exposure modes and 3 lenses. Second, we propose a conventional ISP pipeline to generate good RGB frames as reference. This conventional ISP pipleline performs basic ISP operations, e.g.demosaicing, white balancing, denoising and color space transforming, with a ColorChecker as reference. Third, we classify the existing learnable ISP methods into 3 classes, and select multiple methods to train and evaluate on our new dataset. Lastly, since there is no prior work for reference, we propose a simple event-guided ISP method and test it on our dataset. We further put forward key technical challenges and future directions in RGB-Event ISP. In summary, to the best of our knowledge, this is the very first research focusing on event-guided ISP, and we hope it will inspire the community. The code and dataset are available at: https://github.com/yunfanLu/RGB-Event-ISP.

==> Code-1-MATLAB-ISP.tex <==
\clearpage
\begin{lstlisting}[language=Matlab, caption=MATLAB ISP Code.]
function ans_colors = RGBE_ISP(
    raw_npz_file,
    json_file,
    has_known_colors,
    known_colors,
    gamma)
    % RGBE_ISP: ISP for RGBE data.
    % raw_npz_file: the raw data file.
    % json_file: the json file for color card.
    % has_known_colors: has known colors.
    % known_colors: the known colors.
    % gamma: gamma value.
    fprintf('RGBE_ISP:\n');
    fprintf('   raw_npz_file :%s\n', raw_npz_file);
    fprintf('   json_file    :%s\n', json_file);
    % Read the raw data for black level calibration.
    pth_blcraw = './rawdata/FixedPatternNoise.npy';
    img_blc = readNPY(pth_blcraw);
    img_blc = double(img_blc) / 242.0;
    % get the file name
    [pathstr, file_name, ext] = fileparts(raw_npz_file);
    % Read rge quad raw data.
    % 242 is the max value of the raw data. The raw data is 8bit.
    % 242 = 255 * 0.95. The 0.95 is the saturation level.
    img_quad = readNPY(raw_npz_file);
    img_quad = max(0, min(img_quad, 242));
    img_quad = double(img_quad) / 242.0;
    img_quad = img_quad - img_blc;
    % clip the value to [0, 1]
    img_quad = max(0, min(img_quad, 1));
    [height, width] = size(img_quad);
    % demosaic the quad raw data.
    % This function can be found in the following link.
    % https://www.mathworks.com/matlabcentral/fileexchange/
    % 116085-quadbayer-cfa-modified-gradient-based-demosaicing
    img_rgb = quad_bayer_demosaic_full(
        img_quad, height, width, 'grgb', 0, 0);
    if has_known_colors
        colors = known_colors;
        ans_colors = [];
    else
        vertex_pts = get_color_card_coords_from_json(json_file);
        % check the vertex_pts has 4 points
        if size(vertex_pts, 1) ~= 4
            disp('Error: vertex_pts has not 4 points');
            return;
        end
        % get the colors from the image given 4 points' location
        % The vertex_pts is the 4 points of the color card.
        [colors, coord] = checker2colors(
            img_rgb, [4, 6], 'mode', 'auto',
            'show', false, 'vertex_pts', vertex_pts);
        % save colors to file
        color_file = sprintf('%s/%s_colors.mat', pathstr, file_name);
        save(color_file, 'colors');
        % the colors will be reture value.
        ans_colors = colors
        % check NaN value in colors. if has NaN value, return.
        if any(isnan(colors))
            disp('Error: colors has NaN value');
            fprintf('raw_npz_file: %s\n', raw_npz_file);
            return;
        end
    end
    % white balance
    wb_multipliers = [
        colors(21, 2) / colors(21, 1),
        1.0,
        colors(21, 2) / colors(21, 3)];
    img_wb = img_rgb;
    img_wb(:, :, 1) = img_wb(:, :, 1) * wb_multipliers(1);
    img_wb(:, :, 3) = img_wb(:, :, 3) * wb_multipliers(3);
    img_wb = max(0, min(img_wb, 1));
    % denoise using rgb BM3D with default parameter
    randn('seed', 0);
    sigma = 25;
    [~, img_denoise] = CBM3D(1, img_wb, sigma);
    % color correction.
    % The color card colors are sRGB from 
    % the document of the color card, 
    % treated as groundtruth sRGB under D65
    srgb = [
            112, 76, 60;
            197, 145, 125;
            87, 120, 155;
            82, 106, 60;
            126, 125, 174;
            98, 187, 166;
            238, 158, 25;
            157, 188, 54;
            83, 58, 106;
            195, 79, 95;
            58, 88, 159;
            222, 118, 32;
            25, 55, 135;
            57, 146, 64;
            186, 26, 51;
            245, 205, 0;
            192, 75, 145;
            0, 127, 159;
            43, 41, 43;
            80, 80, 78;
            122, 118, 116;
            161, 157, 154;
            202, 198, 195;
            249, 242, 238;
            ];
    srgb = srgb / 255.0; %normlization
    srgb = srgb .^ 2.2;  %sRGB to linear sRGB
    colors_wb = colors .* wb_multipliers % white balance correction
    % compute the color correction matrix.
    [cam2xyz, scale, ~, ~] = ccmtrain(colors_wb, ...
        srgb, 'omitlightness', true, 'preservewhite', true, ...
        'model', 'linear3x3', 'targetcolorspace', 'sRGB', ...
        'whitepoint', whitepoint('d65'));
    % apply the color correction matrix.
    lin_srgb = apply_cmatrix(
        img_denoise * (scale * 0.9),transpose(cam2xyz));
    lin_srgb = max(0, min(lin_srgb, 1));
    % gamma correction.
    img_srgb = lin_srgb .^ gamma;
    img_srgb = max(0, min(img_srgb, 1));
    good_rgb_file = sprintf(
        '%s/%s_good_rgb.png', pathstr, file_name);
    imwrite(img_srgb, good_rgb_file);
    fprintf('DONE: %s', good_rgb_file);
end
\end{lstlisting}

==> Table-4-NIQE-in.tex <==
\begin{table}[t!]
\centering
\caption{Comparison of Methods on HVS ISP Dataset indoor scenes. $^*$ refer to the results obtained by the same model with different hyperparameters.}

\resizebox{1\linewidth}{!}{
\setlength{\tabcolsep}{0.012\linewidth}{
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
&
\multicolumn{2}{c}{\texttt{1-In-Fruit-2}}
&
\multicolumn{2}{c}{\texttt{3-In-ColChecker-40}}
&
\multicolumn{2}{c}{\texttt{4-In-RLChart-10}}
&
\multicolumn{2}{c}{\texttt{Average}} \\
\textbf{Methods}
& \textbf{NIQE}  & \textbf{PI}
& \textbf{NIQE}  & \textbf{PI}
& \textbf{NIQE}  & \textbf{PI}
& \textbf{NIQE}  & \textbf{PI} \\
\midrule
\textbf{PyNET}
& 10.5604 & 8.9322 & 8.6510 & 7.8808 & 8.6960 & 7.9034 & 9.3024 & 8.2388 \\
\textbf{PyNET$^*$}
& 10.6142 & 9.0591 & 9.5254 & 8.4616 & 9.2743 & 8.2574 & 9.8046 & 8.5927 \\
\textbf{PyNetCA}
& 9.5175  & 8.4227 & 9.5633 & 8.3391 & 10.0280 & 8.4848 & 9.7029 & 8.4155 \\
\textbf{InvertISP}
& 9.6301  & 8.2957 & 7.7260 & 7.2639 & 9.2377  & 8.0033 & 8.8646 & 7.8543 \\
\textbf{MV-ISPNet}
& 10.8919 & 9.2025 & 9.6756 & 8.3477 & 9.3904  & 8.3674 & 9.9859 & 8.6392 \\
\textbf{CameraNet}
& 771.8745 & 392.2881 & 771.8748 & 392.2880 & 771.8735 & 392.2873 & 771.8743 & 392.2878 \\
\textbf{CameraNet$^*$}
& 667.3576 & 335.3488 & 667.356 & 335.3535 & 667.3693 & 335.3525 & 667.3644 & 335.3501 \\
\textbf{AWNet}
& 9.0410  & 8.4831 & 8.8963 & 8.2489 & 7.6562  & 7.2208 & 8.5311 & 7.9843 \\
\textbf{Swin-Transformer}
& 7.8467  & 7.3106 & 7.9101  & 7.2932 & 7.3744 & 7.0336 & 7.7104 & 7.2125 \\
\textbf{UNet}
 & 10.7405 & 9.3207 & 9.7168  & 8.6760 & 9.5778 & 8.5257 & 10.0117 & 8.8408 \\
\textbf{UNet$^*$}
& 11.5525 & 9.9720 & 10.3320 & 9.0237 & 10.7163 & 9.2440 & 10.8669 & 9.4132 \\
\hline
\textbf{eSL}
& 8.9799  & 8.1130 & 8.5955  & 7.8486 & 8.9683  & 8.0099 & 8.8479  & 7.9905 \\
\textbf{EV-UNet}
& 10.3218 & 9.2965 & 10.7447 & 9.1840 & 10.8084 & 9.1588 & 10.6250 & 9.2131 \\


\toprule
\label{table:method_indoor_NIQE_performance}
\end{tabular}
}}

\end{table}



==> Table-5-NIQE-out.tex <==
\begin{table}[t!]
\centering
\caption{Comparison of methods on HVS ISP dataset outdoor scenes. $^*$ refer to the results obtained by the same model with different hyperparameters.}

\resizebox{1\linewidth}{!}{
\setlength{\tabcolsep}{0.012\linewidth}{
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
&
\multicolumn{2}{c}{\texttt{2-OUT-Tree-2}}
&
\multicolumn{2}{c}{\texttt{3-Out-Flower-2}}
&
\multicolumn{2}{c}{\texttt{4-Out-Building-1}}
&
\multicolumn{2}{c}{\texttt{Average}} \\
\textbf{Methods}
& \textbf{NIQE}  & \textbf{PI}
& \textbf{NIQE}  & \textbf{PI}
& \textbf{NIQE}  & \textbf{PI}
& \textbf{NIQE}  & \textbf{PI} \\
\midrule
\textbf{PyNET}
& 8.9608 & 8.2063 & 8.4138 & 7.8977 & 8.0532 & 7.6866 & 8.4759 & 7.9302 \\
\textbf{PyNET$^*$}
& 9.3716 & 8.4749 & 9.2355 & 8.2926 & 9.1500 & 8.2384 & 9.2523 & 8.3353 \\
\textbf{PyNetCA}
& 8.4343 & 7.8880 & 7.9795 & 7.6717 & 7.8525 & 7.6036 & 8.0888 & 7.7211 \\
\textbf{InvertISP}
& 7.5380 & 7.3978 & 6.7139 & 6.9881 & 5.9043 & 6.2299 & 6.7187 & 6.8720 \\
\textbf{MV-ISPNet}
& 8.1110 & 7.8820 & 7.4862 & 7.2422 & 7.4597 & 7.1434 & 7.6856 & 7.4225 \\
\textbf{CameraNet}
& 771.8750 & 392.2857 & 771.8755 & 392.2860 & 771.8743 & 392.2864 & 771.8749 & 392.2860 \\
\textbf{CameraNet$^*$}
& 667.3654 & 335.3526 & 337.3615 & 335.3509 & 667.3656 & 335.3555 & 667.3632 & 335.3525 \\
\textbf{AWNet}
& 8.6385 & 8.3241 & 8.4038 & 8.1231 & 7.0224 & 7.4135 & 8.0216 & 7.9536 \\
\textbf{Swin-Transformer}
& 7.4143 & 7.4885 & 7.2316 & 7.4287 & 6.4391 & 6.7594 & 7.0284 & 7.2255 \\
\textbf{UNet}
& 8.8706 & 8.2537 & 8.2972 & 7.8604 & 8.2363 & 7.7737 & 8.4680 & 7.9626 \\
\textbf{UNet$^*$}
& 8.8747 & 8.2149 & 8.4267 & 7.9218 & 8.4236 & 8.0117 & 8.5750 & 8.0495 \\
\hline
\textbf{eSL}
& 7.8569 & 7.7214 & 6.7929 & 7.0928 & 6.2029 & 6.6194 & 6.9509 & 7.1445 \\
\textbf{EV-UNet}
& 8.5472 & 8.0862 & 8.1830 & 7.8198 & 8.0310 & 7.7055 & 8.2537 & 7.8705 \\

\toprule
\label{table:method_outdoor_NIQE_performance}
\end{tabular}
}}

\end{table}



==> Table-7-In-Out-in-One-Table.tex <==
\begin{table}[t]
\centering
\caption{\small Comparison of Methods on HVS ISP Dataset indoor and outdoor scenes.}
\resizebox{1\linewidth}{!}{
\setlength{\tabcolsep}{0.012\linewidth}{
\begin{tabular}{l ccc ccc ccc}
\toprule
& \multicolumn{3}{c}{\texttt{Out-Average}}
& \multicolumn{3}{c}{\texttt{In-Average}}
& \multicolumn{3}{c}{\texttt{All-Average}} \\
\textbf{Methods}
& \textbf{PSNR}$\uparrow$   & \textbf{SSIM}$\uparrow$  & $L_1$$\downarrow$
& \textbf{PSNR}$\uparrow$   & \textbf{SSIM}$\uparrow$  & $L_1$$\downarrow$
& \textbf{PSNR}$\uparrow$   & \textbf{SSIM}$\uparrow$  & $L_1$$\downarrow$ \\
\midrule
\textbf{PyNET}
& 32.47 & 0.9785 & 0.0180 & 11.97 & 0.7664 & 0.2412 & 22.22 & 0.8725 & 0.1296 \\
\textbf{PyNET$^*$}
& 29.37 & 0.9652 & 0.0265 & 17.36 & 0.8437 & 0.1494 & 23.37 & 0.9044 & 0.0880 \\
\textbf{PyNetCA}
& 31.76 & 0.9762 & 0.0207 & 27.72 & 0.9431 & 0.0540 & 29.74 & 0.9596 & 0.0373 \\
\textbf{InvertISP}
& 27.59 & 0.9364 & 0.0281 & 28.27 & 0.9392 & 0.0254 & 27.93 & 0.9378 & 0.0268 \\
\textbf{MV-ISPNet}
& 29.76 & 0.9662 & 0.0232 & 31.12 & 0.9664 & 0.0207 & 30.44 & 0.9663 & 0.0219 \\
\textbf{CameraNet}
& 11.36 & 0.2618 & 0.2266 & 13.04 & 0.2591 & 0.2013 & 12.20 & 0.2605 & 0.2139 \\
\textbf{CameraNet$^*$}
& 12.30 & 0.3953 & 0.2096 & 12.68 & 0.2672 & 0.2073 & 12.49 & 0.3312 & 0.2085 \\
\textbf{AWNet}
& 17.04 & 0.9180 & 0.0879 & 27.03 & 0.9356 & 0.0567 & 22.04 & 0.9268 & 0.0723 \\
\textbf{Swin-Transformer}
& 25.24 & 0.9463 & 0.0354 & 25.80 & 0.9481 & 0.0304 & 25.52 & 0.9472 & 0.0329 \\
\textbf{UNet}
& 24.51 & 0.9634 & 0.0354 & 15.70 & 0.8913 & 0.1124 & 20.11 & 0.9274 & 0.0739 \\
\textbf{UNet$^*$}
& 28.17 & 0.9685 & 0.0265 & 31.76 & 0.9705 & 0.0188 & 29.97 & 0.9695 & 0.0226 \\
\textbf{eSL-Net}
& 23.02 & 0.9294 & 0.0473 & 26.13 & 0.9464 & 0.0381 & 24.57 & 0.9379 & 0.0427 \\
\textbf{EV-UNet}
& 30.11 & 0.9698 & 0.0225 & 26.04 & 0.9388 & 0.0640 & 28.08 & 0.9543 & 0.0432 \\
\bottomrule
\label{table:method_indoor_outdoor_performance}
\end{tabular}
}}
\end{table}

